Parallel and Streaming Algorithms for K-Core Decomposition

The $k$-core decomposition is a fundamental primitive in many machine learning and data mining applications. We present the first distributed and the first streaming algorithms to compute and maintain an approximate $k$-core decomposition with provable guarantees. Our algorithms achieve rigorous bounds on space complexity while bounding the number of passes or number of rounds of computation. We do so by presenting a new powerful sketching technique for $k$-core decomposition, and then by showing it can be computed efficiently in both streaming and MapReduce models. Finally, we confirm the effectiveness of our sketching technique empirically on a number of publicly available graphs.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	sample-manuscript.tex \
	sample-acmsmall.tex \
	sample-acmlarge.tex \
	sample-acmtog.tex \
	sample-sigconf.tex \
	sample-sigconf-authordraft.tex \
	sample-sigplan.tex \
	sample-sigchi.tex \
	sample-sigchi-a.tex 


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do 	pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf sample-*.pdf


==> conc_1.tex <==
\section{Conclusions and future works}
In this paper we introduce a new sketching technique for computing the core-labeling of a graph. Using this new technique, we design efficient MapReduce and streaming algorithms to approximate the coreness number of all the nodes in a graph efficiently. We also confirm the effectiveness of  our sketch via an empirical study.
The most interesting open problem in the area is to design a fully dynamic algorithm~\cite{italiano1999dynamic} to maintain the core-labeling of a graph by using only $\polylog n$ operations per update(edge addition or deletion).

==> fig/stats/_Rhistory <==
data <- read.table("scalability", header=F, sep="\t")
data <- read.table("scalability", header=F, sep="\t")
q
quit
q()
data <- read.table("scalability", header=F, sep="\t")
q()


==> turnstile.tex <==
\subsection{Turnstile algorithms}

Here we show an application of our sketch in the turnstile setting, where we have both addition and deletion of the edges. 

We use $t$-sparse recovery data structures defined as follow to handle deletions. There are algorithms that provide $t$-sparse recovery data structures using $\tilde{O}(t)$ space~\cite{barkay2015efficient}.

\begin{definition}
	 A $t$-sparse recovery data structure is a data structure which handles insertions and deletions of elements and if the current number of elements stored in it is at most $t$, then these elements can be recovered.
\end{definition}

To handle deletions, in addition to the data structure used for the addition-only streaming algorithm, for each graph $H_j$ and each $v$ vertex in $H_j$ we keep a $\frac{24\log n}{\epsilon^2}$-sparse recovery data structure $S^v_j$. Upon insertion of each edge $(u,v)$ if it is sampled in the $j$-th iteration (passed Line~\ref{line:probIf} of Algorithm~\ref{Alg:turnstile}) and is not inserted in $H_j$ (i.e., failed Line~\ref{line:lambdaIf} of Algorithm~\ref{Alg:turnstile}), we insert $(u,v)$ to $S^u_j$ and $S^v_j$.

Upon deleting an edge $(u,v)$ we need to remember the random number $r$ that we used for $(u,v)$ previous time. To do this we simply use $\tilde{O}(n)$-minwise independent hash functions~\cite{feigenblat2011exponential} and hash $(u,v)$ to get its corresponding random number. The pseudo-code our algorithm in the turnstile setting is presented in Algorithm~\ref{Alg:turnstile}.

Following is the procedure to delete an edge $(u,v)$. For each $H_j$ if $(u,v)\in H_j$ we remove $(u,v)$ from $H_j$. Otherwise, if $(u,v)$ is sampled in the $j$-th iteration, it means that it is inserted into $S^u_j$ and $S^v_j$. In this case we delete $(u,v)$ from $S^u_j$ and $S^v_j$. Next, we recompute $\Lambda_{j}$, and denote it by $\Lambda_{j}^{new}$\footnote{Indeed, one could recompute $\lambda_{j'}$ for any choice of $j'$. However, we note that this recomputation does not affect a $\lambda_{j'}$ with $j' < j$, and the recomputation will happen for a $\lambda_{j'}$ with $j'>j$ by the iteration in Line \ref{line:for}}. 
Let $\Lambda_j^{\Delta} = \Lambda_{j} - \Lambda_{j}^{new}$ be the sequence of vertices that are removed from $\Lambda_{j}$ after this recomputation, ordered by their removal order in the greedy algorithm (See Line \ref{line:delta}). We iterate over the vertices in $\Lambda_j^{\Delta}$ and recover their edges (See Line \ref{line:recover}). 
%
Remember that the edges in $S_j^{v'}$ are those that both their endpoints fall in $Lambda_j$. Let $\Lambda_j^{\Delta} =\{v'_1,v'_2,v'_3,\dots,v'_{\Delta}\}$ be the sequence vertices that move out of $\Lambda_j$ as we remove $(u,v)$, and assume $v'_1,v'_2,v'_3,\dots,v'_{\Delta}$ is in the same order that the greedy algorithm (in Line \ref{line:greedy}) removes these vertices. Recall that, if a vertex is not in $\Lambda_j^{new}$ its label assigned by the greedy algorithm is at most $\frac{24\log n}{\epsilon^2}$ (due to Line \ref{line:lj}). Thus, upon removal of $v'_1$ the number of edges between $v'_1$ and [the old] $Lambda_j$ is at most $\frac{24\log n}{\epsilon^2}$. Thus, we can recover all of the edges of $v'_1$. Similarly note that, when greedy is removing $v'_2$ the number of edges between $v'_2$ and $Lambda_j - \{v_1 \}$  is at most $\frac{24\log n}{\epsilon^2}$. Note that after recovering $S_j^{v'_1}$ we observe if there is an edge between $v'_1$ and $v'_2$ or not, and we removed it from $S_j^{v'_2}$. Thus, $S_j^{v'_2}$ only contains the edges between $v'_2$ and $\Lambda_j - \{v_1 \}$ which is upper bounded by $\frac{24\log n}{\epsilon^2}$. Hence we can recover the edges in $S_j^{v'_2}$. The same argument holds for $v_3$ and so on.

By the results presented in the previous section
we obtain the following corollary.

\begin{corollary}\label{cor:streaming}
	There exists a turnstile algorithm that computes an approximate core-labeling of the input graph using $\tilde{O}(n)$ space.
\end{corollary}


\begin{algorithm}
	\small
	\KwInput{A sequence of insertions and deletions of the edges of the input graph $G(V,E)$ with $n$ vertices and parameter $\epsilon \in (0,1]$.}\;
	\vspace{0.3cm}
	\bf{Initialization:}\\
	\For{$j = 0$ to $\log n$}{
		 $\Lambda_j \leftarrow \emptyset$\;
		 $H_j \leftarrow (V,\emptyset)$\;
		 $p_j \leftarrow 2^j \frac{12 \log n}{\epsilon^2 n}$\;
		\For{$v \in V$}{
			Initiate a $\frac{24\log n}{\epsilon^2}$-sparse recovery $S^v_j \leftarrow \emptyset$\;
		}
	}
	 $\Lambda_{-1} \leftarrow \emptyset$\;
	 Let $h(u,v): (V,V)\rightarrow [0,1]$ be a $\tilde{O}(n)$-minwise independent hash function.

	\vspace{0.3cm}
	 \bf{Insertion of $(u,v)$}\;
	$r \leftarrow h(u,v)$\; 
	\For{$j = 0$ to $\log n$}{
		\If{$r\leq p_j$}{\label{line:probIf}
			\If{$v\notin\Lambda_{j-1}$ or $u \notin \Lambda_{j-1}$}{\label{line:lambdaIf}
				Add $(u,v)$ to $H_j$\;
				Run $Exclusive\_Core\_Labeling(H_j,\Lambda_{j-1})$ and denote the label of vertex $i$ on $H_j$ by $l_j(i)$\; 
				$\Lambda_{j}\leftarrow \emptyset$\;
				\For{$i \in H_j$}{
					\If{$l_j(i) \geq \frac{24\log n}{\epsilon^2} \vee p_j = 1$}{
						%// Node $i$ has sufficiently high degree to estimate its coreness number.\\
						\If{$l_j(i) \leq \frac{48\log n}{\epsilon^2}$}{
							Set the label of vertex $i$ to $(1-\epsilon)\frac{l_j(i)}{p_j}$\;
							Add $i$ to $\Lambda_{j}$\;
						}\Else{
							Set the label of vertex $i$ to $ \frac{2(1-\epsilon)n}{2^{j-1}}$\;
							Add $i$ to $\Lambda_{j}$\;
						}
					}
				}
			Remove any edge in $H_{j+1}$ induced by $\Lambda_j$\;
		}\Else{
			Add $(u,v)$ to $S^u_j$\;
			Add $(u,v)$ to $S^v_j$\;
		}
	}
	}




\vspace{0.3cm}
\bf{Deletion of $(u,v)$}\;
$r \leftarrow h(u,v)$\; 
\For{$j = 0$ to $\log n$}{\label{line:for}
	\If{$r\leq p_j$}{
		\If{$v\notin\Lambda_{j-1}$ or $u \notin \Lambda_{j-1}$}{
			Delete $(u,v)$ from $H_j$\;
			Run $Exclusive\_Core\_Labeling(H_j,\Lambda_{j-1})$ and denote the label of vertex $i$ on $H_j$ by $l_j(i)$\;\label{line:greedy}
			$\Lambda_{j}^{new}\leftarrow \emptyset$\;
			\For{$i \in H_j$}{
				\If{$l_j(i) \geq \frac{24\log n}{\epsilon^2} \vee p_j = 1$}{\label{line:lj}
					%// Node $i$ has sufficiently high degree to estimate its coreness number.\\
					\If{$l_j(i) \leq \frac{48\log n}{\epsilon^2}$}{
						Set the label of vertex $i$ to $(1-\epsilon)\frac{l_j(i)}{p_j}$\;
						Add $i$ to $\Lambda_{j}^{new}$\;
					}\Else{
						Set the label of vertex $i$ to $ \frac{2(1-\epsilon)n}{2^{j-1}}$\;
						Add $i$ to $\Lambda_{j}^{new}$\;
					}
				}
				Let $\Lambda_j^{\Delta} \leftarrow \Lambda_{j} - \Lambda_{j}^{new}$ ordered by the removal oreder in Line \ref{line:greedy}\;\label{line:delta}
				\For{$v'\in \Lambda_j^{\Delta}$}{\label{line:recover}
					Recover $S^{v'}_j$\;
					Add the edges in $S^{v'}_j$ to $H_j$\;
					Remove all the edges in $S^{v'}_j$ from the sparse recovery of both their endpoints\;
				}
				$\Lambda_{j} \leftarrow \Lambda_{j}^{new}$\;
			}
		}\Else{
			Delete $(u,v)$ from $S^u_j$\;
			Delete $(u,v)$ from $S^v_j$\;
		}
	}
}

	
	\caption{\small An algorithm to compute $1-O(\epsilon)$ approximate core-labeling in the turnstile setting.}
	\label{Alg:turnstile}
\end{algorithm}




